SKED: Sketch-guided Text-based 3D Editing

Text-to-image diffusion models are gradually introduced into computer graphics, recently enabling the development of Text-to-3D pipelines in an open domain. However, for interactive editing purposes, local manipulations of content through a simplistic textual interface can be arduous. Incorporating user guided sketches with Text-to-image pipelines offers users more intuitive control. Still, as state-of-the-art Text-to-3D pipelines rely on optimizing Neural Radiance Fields (NeRF) through gradients from arbitrary rendering views, conditioning on sketches is not straightforward. In this paper, we present SKED, a technique for editing 3D shapes represented by NeRFs. Our technique utilizes as few as two guiding sketches from different views to alter an existing neural field. The edited region respects the prompt semantics through a pre-trained diffusion model. To ensure the generated output adheres to the provided sketches, we propose novel loss functions to generate the desired edits while preserving the density and radiance of the base instance. We demonstrate the effectiveness of our proposed method through several qualitative and quantitative experiments. https://sked-paper.github.io/

==> figs/fig_res_qual_multi_letter.tex <==
\begin{figure}
\centering
  \includegraphics[width=0.99\columnwidth]{data/results_multi_letter.png}
  \caption{Generating logos utilizing multiple letters.}
  \label{fig:res_qual_multi_letter}
\end{figure}

==> tables/tab_ablation.tex <==
\begin{table}
	\centering
	\begin{tabular}{lrrr}
	\toprule
        Method & FID$\downarrow$ & OCR$\uparrow$ & CLIP $\uparrow$    \\
		\midrule
         w/o Dis   &  &  &  \\
         w/o mask &  &   &   \\
         w/o $l_{rec}$ &  &  &    \\
         Ours  &  &    & \\
		\bottomrule
	\end{tabular}

  	\caption{Abaltion Studies.}

    \label{tab:ablation}
\end{table}


==> tables/tab_bkup.tex <==

% \begin{table}
% \centering
% % \setlength{\tabcolsep}{4pt}

% \caption{\textbf{PSNR}: is measured against renderings from the base model, to asses the method's ability to preserve the original content. }
% \label{tab:psnr_clipsim}

% % \footnotesize
% \begin{tabular}{l \tsm l \ts c \ts c \tsm c \ts c  \tsm c \ts c}
% \toprule

% {Method} & {Model} & \multicolumn{2}{c  \tsm  \ts}{{PSNR $\uparrow$}}  & \multicolumn{2}{c \tsm}{{CLIP-Sim $\uparrow$}} \\ 


% && View A & View B
% & View A & View B \\
%  \midrule
%  \ours  & Horse 
%  & \textbf{1.64} &  \textbf{9.9}
%  & \textbf{7.03} & \textbf{12.3}\\

%  \ours  & Flower 
%  & \textbf{1.64} &  \textbf{9.9}
%  & \textbf{7.03} & \textbf{12.3}\\

%  \ours  & Cupcake
%  & \textbf{1.64} &  \textbf{9.9}
%  & \textbf{7.03} & \textbf{12.3}\\

%  \ours  & Sundae
%  & \textbf{1.64} &  \textbf{9.9}
%  & \textbf{7.03} & \textbf{12.3}\\

%  \ours  & Cat 
%  & \textbf{1.64} &  \textbf{9.9}
%  & \textbf{7.03} & \textbf{12.3}\\

%  \ours  & Mean 
%  & \textbf{1.64} &  \textbf{9.9}
%  & \textbf{7.03} & \textbf{12.3}\\
 
% Text-only & Horse
% & 2.06 & 12.9
% & 7.55 & 14.0 \\

% Text-only & Flower
%   & 2.06 & 12.9
%   & 7.55 & 14.0 \\

%   Text-only & Cupcake
%   & 2.06 & 12.9
%   & 7.55 & 14.0 \\

%   Text-only & Sundae
%   & 2.06 & 12.9
%   & 7.55 & 14.0 \\

%   Text-only & Cat 
%   & 2.06 & 12.9
%   & 7.55 & 14.0 \\

%   Text-only & Mean
%   & 2.06 & 12.9
%   & 7.55 & 14.0 \\

% \bottomrule

% \end{tabular}


% \end{table}



==> tables/tab_eval_quan.tex <==
\begin{table}
	\centering
	\begin{tabular}{lrrrr}
	\toprule
        Method & FID$\downarrow$ & OCR$\uparrow$ & CLIP $\uparrow$  & User $\uparrow$  \\
		\midrule
         SD~\cite{rombach2022high}  &  &  &  \\
         CLIPDraw~\cite{frans2021clipdraw} &  &   &   \\
         DF-GAN~\cite{wang2022diffusion} &  &  &    \\
         Ours  &  &    & \\
		\bottomrule
	\end{tabular}

  	\caption{Quantitative comparisons to the related methods.}

    \label{tab:eval_quan_abc}
\end{table}
